EQFace: A Simple Explicit Quality Network for Face Recognition

As the deep learning makes big progresses in still-image face recognition, unconstrained video face recognition is still a challenging task due to low quality face images caused by pose, blur, occlusion, illumination etc. In this paper we propose a network for face recognition which gives an explicit and quantitative quality score at the same time when a feature vector is extracted. To our knowledge this is the first network that implements these two functions in one network online. This network is very simple by adding a quality network branch to the baseline network of face recognition. It does not require training datasets with annotated face quality labels. We evaluate this network on both still-image face datasets and video face datasets and achieve the state-of-the-art performance in many cases. This network enables a lot of applications where an explicit face quality scpre is used. We demonstrate three applications of the explicit face quality, one of which is a progressive feature aggregation scheme in online video face recognition. We design an experiment to prove the benefits of using the face quality in this application. Code will be available at \url{https://github.com/deepcam-cn/facequality}.

==> content/backup.tex <==
Face recognition, as one classical task in computer vision, has made tremendous advancements with the help of deep CNN. The first step of face recognition is to detect a face in an still or video image. Then a feature vector is extracted to represent the face image. The distance between feature vectors of two face images is defined as the similarity of these two faces, and is used to verify or recognize a face image. It is expected that the distance between face images of a same person or class is smaller than that between faces images of two different persons or classes. 

Currently, the focus of face recognition is to increase the discrimination capability of a model by decreasing the distance inside a class and increasing the distance between classes.  To achieve this goal, there are three directions. 

The first one is to expand and clean data sets. For face recognition, a better data set has an noticeable effect on face recognition performance. The publication of data sets like VGGFace2\cite{Cao18}, MS1M\cite{ms1m} helps significantly improve the face recognition performance. 

The second one is to optimize the loss function. In same condition, different loss function shows big influence on face recognition performance. Recently, new loss functions including SphereFace\cite{SphereFace}, CosFace\cite{CosFace}, ArcFace\cite{SphereFace}, CircleLoss\cite{sun2020circle} have been proposed.  

The last one is the optimization of the backbone network.  It is critical to 
design a backbone network that can have a good trade-off between speed and performance, 
particularly in cases where the hardware’s computing power is limited. Along this direction, the MobileFaceNets\cite{MobileFaceNets}, VarGFaceNet\cite{VarGFaceNet}, 
SeesawFaceNets\cite{zhang2019seesawfacenets} have been proposed.

Quite a few approaches have been studied to combat this problem including \cite{Noise1},\cite{Noise2},\cite{Noise3},\cite{Noise4},\cite{Noise5}.  Our idea is along the line of reweighting with a face quality, if it is explicitly available. As pointed out in \cite{Subcenter}, re-weighting methods are susceptible to the performance of the initial model. We work around this problem by proposing an iterative training pipeline. In \cite{WangNoise}, a co-mining strategy using the loss values as the cue to simultaneously detect noisy labels, exchange the high-confidence clean faces to alleviate the error accumulation caused by the sampling bias, and re-weight the
predicted clean faces to make them dominate the discriminative model training. However, the co-mining method requires training twin networks simultaneously and it is
challenging to train large networks (e.g. ResNet100 [10]) on a large-scale dataset (e.g.
MS1M [9] and Celeb500K [1]).


Our second contribution is that we propose a progressive feature aggregation using the face quality score out of the QFQN for on-the-fly video face recognition. Unlike in the bench-marking protocol of YTF and IJB data sets, where feature aggregation is done after all video frames are processed, we aggregate the features on-the-fly while video frames are processed. This is close to the video face recognition in practical deployment. 

In order to compare with the video face recognition results other researchers benchmarked on the YTF and IJB data sets, we modified our aggregation scheme for the bench marking purpose. We evaluate the performance on the video face data sets YTF and IJB and show the performance improvement.  

Lastly we design an experiment to evaluate the performance of the progressive feature aggregation in on-the-fly video face recognition. Our results show the impressive improvement from this aggregation scheme using QFQN quality score. 



\begin{table*}
  \centering
  \caption{1:1 verification (Vrf) and 1:N identification (Idt) performance (\%) on IJB-B, IJB-C datasets.}
  \begin{tabular}{|l|l|l|l|l|l|l|l|l}
    \hline
    \multirow{2}{*}{Method} &
      \multicolumn{2}{c}{IJB-B Vrf} &
      \multicolumn{2}{c}{IJB-B Idt} &
      \multicolumn{2}{c|}{IJB-C Vrf} & 
      \multicolumn{2}{c|}{IJB-C Idt} \\
    & FAR=1E-5  & FAR=1E-4 & Rank1 & Rank5 & FAR=1E-5  & FAR=1E-4 & Rank1 & Rank5 \\
    \hline
    ArcFace \cite{ArcFace} & 89.21 &  94.23 &  95.14  & 96.85 &  93.5 &  95.8  & 95.87 & 97.27 \\
    URFace \cite{journals/corr/abs-2002-11841} & - &  -  &  - & -  & 95.0 & 96.6 & 96.00 & 97.06 \\
    \hline
    Ours (QW)  & - & -  & - & - & 53.08 & 91.27 & - & -\\
    Ours (QWFA)  & 81.94 & 94.68  & - & - & 91.84 & 96.17 & - & -\\
    Ours (QWFA on ArcFace)   & - & -  & - & - & 53.08 & 91.27 & - & -\\
    Ours (QWFAF on ArcFace)  & 81.94 & 94.68  & - & - & 91.84 & 96.17 & - & -\\


    \hline
  \end{tabular}
  \label{IJB}
\end{table*}


\begin{table*}[ht]
    \centering
    \caption{Verification performance (\%) using face quality filter in training data on LFW, CALFW, CPLFW, CFP\_FP, and YTF.}
    \begin{tabular}{c|c|c|c|c|c}
        \hline
        Method & LFW\cite{LFWTech} & CALFW\cite{CALFW} & CPLFW\cite{CPLFWTech} &  CFP\_FP\cite{cfp-paper} & YTF  \\
        \hline
        Baseline & 99.80 & 95.91 & 92.55 & 98.34 & - \\
        QW & 99.82 & \textbf{95.98} & \textbf{92.60} & 98.20 & 98.02\\
        QWDF,$s_{th}$=0.1 & -  &  -  &  - &  - & 98.12\\
        QWDF,$s_{th}$=0.2 & -  &  -  &  - &  - & 98.12\\
        QWDF,$s_{th}$=0.3 & -  &  -  &  - &  - & 98.12\\
        \hline
    \end{tabular}
    \label{quality_in_training}
\end{table*}

